The Effect of Modeling Human Rationality Level on Learning Rewards from Multiple Feedback Types

When inferring reward functions from human behavior (be it demonstrations, comparisons, physical corrections, or e-stops), it has proven useful to model the human as making noisy-rational choices, with a "rationality coefficient" capturing how much noise or entropy we expect to see in the human behavior. Prior work typically sets the rationality level to a constant value, regardless of the type, or quality, of human feedback. However, in many settings, giving one type of feedback (e.g. a demonstration) may be much more difficult than a different type of feedback (e.g. answering a comparison query). Thus, we expect to see more or less noise depending on the type of human feedback. In this work, we advocate that grounding the rationality coefficient in real data for each feedback type, rather than assuming a default value, has a significant positive effect on reward learning. We test this in both simulated experiments and in a user study with real human feedback. We find that overestimating human rationality can have dire effects on reward learning accuracy and regret. We also find that fitting the rationality coefficient to human data enables better reward learning, even when the human deviates significantly from the noisy-rational choice model due to systematic biases. Further, we find that the rationality level affects the informativeness of each feedback type: surprisingly, demonstrations are not always the most informative -- when the human acts very suboptimally, comparisons actually become more informative, even when the rationality level is the same for both. Ultimately, our results emphasize the importance and advantage of paying attention to the assumed human-rationality level, especially when agents actively learn from multiple types of human feedback.

==> [Ghosal][AAAI'22] The Effect of Modeling Human Rationality Level on Learning Rewards from Multiple Feedback Types AAAI (1)/sup.tex <==

% \section{Appendix}
\onecolumn

\section{Expected Information Gain of Design}\label{app:infogain_derivation}
In actively selecting over feedback types, we evaluate feedback designs $x \in \mathcal{X}$ by expected information gain from querying the human for feedback $x$. In Table~1, we provide a reference of the different feedback types, their designs, and choice sets. Concretely active learning over feedback types can be written as:
\begin{equation*}
        \max_{x \in \mathcal{X}} \mathbb{E}_{y \sim P(y|x})[D_{KL}(P(\theta | y, x)||P(\theta)]
\end{equation*}
Using the definition of the KL-Divergence, we have that
\begin{align*}
    \mathbb{E}_{y \sim P(y|x})[D_{KL}(P(\theta | y, x)||P(\theta)]\\ = \mathbb{E}_{y \sim P(y|x)} [\mathbb{E}_{\theta \sim P(\theta|y,x)}[\log P(\theta|y,x) - \log P(\theta)]]\\
    = \mathbb{E}_{y \sim P(y|x)}[-H(P(\theta|y,x))- \mathbb{E}_{\theta \sim P(\theta|y,x)}[\log P(\theta)]]\\
    = \mathbb{E}_{y \sim P(y|x)}[-H(P(\theta|y,x))] - \mathbb{E}_{\theta, y \sim P(\theta, y|x)}[\log P(\theta)]\\
    = \mathbb{E}_{y \sim P(y|x)}[-H(P(\theta|y,x))] + H(P(\theta))\\
    = \mathbb{E}_{y\sim P(y|x)}[H(P(\theta))-H(P(\theta|y,x)]
\end{align*}
Furthermore, we wish to avoid calculating the posterior distribution $P(\theta|y,x)$ since we do not explicitly have access to this distribution. By expanding the entropy term 
\begin{align*}
    \mathbb{E}_{y \sim P(y|x)}[\mathbb{E}_{\theta \sim P(\theta|y,x)}[\log \frac{P(\theta|y,x)}{P(\theta)}]]\\ = \mathbb{E}_{y,\theta \sim P(y,\theta|x)}[\log \frac{P(\theta|y,x)}{P(\theta)}]\\ 
    = \mathbb{E}_{y,\theta \sim P(y,\theta|x)}[\log \frac{P(\theta|y, x)}{P(\theta|x)}]\\
    = \mathbb{E}_{y, \theta \sim P(y,\theta|x)}[\log \frac{P(y|x,\theta)}{P(y|x)}]\\
    = \mathbb{E}_{\theta \sim P(\theta|x)}[\mathbb{E}_{y \sim P(y|x,\theta)}[\log \frac{P(y|x,\theta)}{P(y|x)}]]\\
    = \mathbb{E}_{\theta \sim P(\theta|x)}[\mathbb{E}_{y \sim P(y|x,\theta)}[\log \frac{P(y|x,\theta)}{\sum\limits_{\hat{\theta}}P(y|x,\theta) P(\theta|x)}]]
\end{align*}
Thus, we see that this can be computed given the set of $\theta$ and the observation model for the human feedback $P(y|x,\theta)$ which are both available explicitly.

We observe that this expression is in terms of the observation model for the human feedback $P(c_h|x, \theta)$, along with the prior $P(\theta)$. In the case of comparisons and e-stops, the inner expectation can be computed exactly due to the small space of feedback that may be received from the human. In the case of demonstrations, we approximate the inner expectation by sampling a small number of demonstrations for each possible pair $(x, \theta)$.

\begin{table*}
\label{tab:feedbacktypes}
\footnotesize
\centering
    \caption{Example feedback types and groundings.}\label{tab:feedback_types}
\begin{tabular}{llll}
\toprule % from booktabs package
\bfseries Feedback Type  & \bfseries Possible Designs $\mathcal{X}$   & \bfseries Choice Set $\mathcal{C}(x)$  & \bfseries Grounding $\varphi(x, c)$ \\
 & & for $x \in \mathcal{X}$ &for $x \in \mathcal{X}, c \in \mathcal{C}(x)$   \\
 \midrule % from booktabs package
            %   &                                & for $x \in \mathcal{X}$                        & for $x \in \mathcal{X}, c \in \mathcal{C}(x)$                                           \\
% Demonstration (old) & Starting states:               & Trajectories:                  & $\varphi(s, \xi) = \xi$    \\
%               & $\mathcal{X} = \mathcal{S}$    & $\mathcal{C}(s) = \{\xi \in \Xi : \xi_0 = s\}$ &                                                                                         \\
% \midrule
              
Demonstration & Starting states:               & Available actions:                  & $\varphi(s, a) = ((s,a))$    \\
              & $\mathcal{X} = \mathcal{S}$    & $\mathcal{C}(s) = \mathcal{A}$ &                                                                                         \\
              
\midrule % from booktabs package

Comparison    & \makecell[l]{Pairs of trajectories:\\ $\mathcal{X} =  \Xi^2$}         & \makecell[l]{Which trajectory:\\   $\mathcal{C}((\xi_A, \xi_B)) = \{A, B\}$   }                              & $\varphi((\xi_A, \xi_B), c) = \begin{cases} \xi_A, & c = A \\ \xi_B, & c = B \end{cases}$ \\

\midrule % from booktabs package
E-Stop        &      \makecell[l]{Trajectories: \\ $\mathcal{X} = \Xi$}                          & \makecell[l]{Stopping time: \\ $C(\xi) = \{0, \ldots, T  \}$}                                     &    $\varphi(\xi,t) = \xi_{0:t}$     \\                                                          \bottomrule % from booktabs package                     
\end{tabular}
\end{table*}
\section{Experimental Setup}\label{app:gridworld}
\subsection{Environment Details}
\begin{figure*}
    \centering
    \includegraphics[width=0.3\textwidth]{NeurIPS/figs/Appendix_Environment.png}
    \caption{\textbf{Example Colored Grid-world Environment.} Here we show an example environment where our user study and simulation experiments take place. The black circle represents the position of the agent and the black bottom-right corner square shows the goal-state. All other tiles have one of four colors.}
    \label{fig:appendixenvironment}
\end{figure*}
Our user study and simulation experiments take place in a 10 by 10 colored grid-world environment, with each tile having one of four colors and the bottom-right corner being a terminal goal state. An example is shown in Figure \ref{fig:appendixenvironment}. We consider a space of reward functions that assign each tile color to a reward earned for landing on that color. For simplicity, we consider the space of normalized reward functions; the reward functions have unit $\ell_{2}$ norm when considered as four-dimensional vectors $\begin{bmatrix}R_{\textrm{red}} \\ R_{\textrm{blue}}\\R_{\textrm{green}}\\ R_{\textrm{yellow}} \end{bmatrix}$. 


\subsection{Reward Inference Performance Metrics}
In this work, we consider two metrics for the success of reward inference metric, as described below: Here $R_{\textrm{inferred}}$ refers to the posterior mean reward and $\theta_{\textrm{inferred}}$ refers to the posterior mean reward vector.\\
\paragraph{Reward Regret} The final goal of reward inference is often to train an agent to maximize the human's reward function. In this setting, the actual values of the reward parameters are irrelevant so long as they induce a similar optimal behavior to the ground-truth reward function. We measure the \textbf{normalized regret}-the amount of reward the agent misses by following the inferred reward- as:
\begin{equation}
\textrm{Regret} = 1-\frac{R_{\textrm{inferrd}}-R_{\textrm{random}}}{R_{\textrm{true}}-R_{\textrm{random}}}
\end{equation}
where $R_{\textrm{inferred}}$ is the reward attained by the optimal policy of the inferred reward under the ground truth reward, $R_{\textrm{random}}$ is the reward attained by a random policy under the ground-truth reward, and $R_{\textrm{True}}$ is the reward attained by the ground-truth reward under the ground-truth reward. 
\paragraph{Reward MSE} Alternatively, we might be interested in how closely the inferred reward parameters match those of the ground-truth. In order to measure this, we computed a reward mean squared error by treating the reward functions as vectors in $\theta \in \mathbb{R}^{4}$, $\theta = \begin{bmatrix} R^{\theta}_{\textrm{red}} \\ R^{\theta}_{\textrm{blue}}\\R^{\theta}_{\textrm{green}}\\R^{\theta}_{\textrm{yellow}} \end{bmatrix}$. Then, we can compute \textbf{reward mean-squared-error} as:
\begin{equation}
    \textrm{MSE} = ||\theta_{\textrm{inferred}} - \theta_{\textrm{ground-truth}}||_{2}^{2}
\end{equation}
In the main text of the paper, we focused on the normalized regret metric, but as we show in the Appendix, our observations correlate well to the reward MSE in general.
\paragraph{Error Bars}
All error bars and ribbons corresponded to the standard error of the mean (SEM). The simulation results have the average and standard error of the mean computed over 10 random reward functions and 2 seeds. The user study results have the average and standard error of the mean computed over the 35 trials performed over 7 subjects.


\subsection{Hyperparameters}
For all simulated experiments, we used the same hyper-parameter settings. All trajectories took place on a 10-by-10 Grid-world with a 4-dimensional reward vector, all lying on the unit sphere. There was a 0.1 transition noise present in the environment. For the purposes of maintaining distributions over reward functions, we discretized this unit sphere by a grid of 1000 points. All experiments were averaged over 10 random seeds.


\section{Reward Inference for Boltzmann Rational Human Feedback}\label{app:other_perf_metrics}
In the main text of the paper, we measured the performance of reward inference using the normalized reward regret. However, another metric we can measure reward inference performance with is the mean-squared error (MSE) when considering the reward functions as four-dimensional vectors. In Figure \ref{fig:app_boltzmannfeedback_mse}, we provide the results of beta-fitting using simulated Boltzmann-rational feedback using this MSE metric. We observe that the mean-squared error metric follows the same general trends as the regret seen in the main text. One important exception, however, is that in the case where we underestimate $\beta$, the MSE results show default having a higher MSE, whereas the regret continues to perform comparably to the fitted and oracle methods. We attribute this to the fact that shifting a reward function by a constant can result in the same eventual behavior, but a reward function whose entries are very different from the ground-truth.


\begin{table*}
\label{tab:feedbacktypeserror}
\footnotesize
\centering
    \caption{Mean Error in Fitting Beta for Different Feedback Types.}\label{tab:menerror}
\begin{tabular}{llll}
 \toprule % from booktabs package
\bfseries Feedback Type  & \bfseries Beta Fit Error   \\
 \midrule % from booktabs package
            %   &                                & for $x \in \mathcal{X}$                        & for $x \in \mathcal{X}, c \in \mathcal{C}(x)$                                           \\
% Demonstration (old) & Starting states:               & Trajectories:                  & $\varphi(s, \xi) = \xi$    \\
%               & $\mathcal{X} = \mathcal{S}$    & $\mathcal{C}(s) = \{\xi \in \Xi : \xi_0 = s\}$ &                                                                                         \\
% \midrule
              
Demonstration & 0.054                                                                       \\
              
\midrule % from booktabs package

Comparison & 0.06 \\

\midrule % from booktabs package
E-Stop  & 0.048                 
\end{tabular}
% \adnote{comparisons -- any two trajectories, or any two trajectoires that start at the same state?; stopping time: the trajectory stays stopped after t, so it repeats xi(t) until the end of the horizon but has the same length, right?;  }

% \dbnote{I don't think there is anything in our formalism requires the trajectories to start from the same point. Our version of e-stops doesn't repeat the stopped state but just ends the episode upon an e-stop.}
\end{table*}
We also tested the accuracy of the beta fitting procedure across the different feedback types and show the results in Table 2. These results demonstrate that our beta-fitting procedure is highly accurate, and this accuracy explains the benefits seen by fitting beta in our paper.
\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/figs/Appendix_demomse.png}
         \caption{Demonstrations}
         \label{subfig:demorational}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/figs/Appendix_msecomp.png}
         \caption{Comparisons}
         \label{subfig:comprational}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/figs/Appendix_estopmse.png}
         \caption{E-Stops}
         \label{subfig:estoprational}
     \end{subfigure}
     \caption{\textbf{Reward MSE on Simulated Boltzmann-Rational Feedback.} We compare the rationality-fitting (Fitted) method which learns $\hat{\beta}$ from data to a Default method which assumes $\hat{\beta}=1$ and an Oracle method which sets $\hat{\beta} = \beta^*$ using the reward mean-squared error metric. Our results generally mirror those using the regret, showing that Fitted (our approach) significantly outperforms Default, achieving similar performance to Oracle. Note that due to the overlap between fitted (orange) and oracle (purple) both curves appear red.}
    \label{fig:app_boltzmannfeedback_mse}
\end{figure*}




% \section{Analysis of Under- and Over-Estimating Beta}\label{app:proofs}

% In \figref{fig:boltzmannfeedback}, we observe an asymmetry between the roles of over- and under-estimating $\beta$. We see that while over-estimation results in poorer performance, under-estimation does not harm reward inference performance as much. In what follows, we present some intuition for this phenomenon. In particular, we show that using a lower $\hat{\beta}$ is risk-averse when the person is suboptimal but is still a good choice even if the person is optimal, whereas a high value of $\hat{\beta}$ leads to the wrong inference when the person is suboptimal. To simplify notation, we define $r(c) \triangleq \mathbb{E}_{\xi \sim \varphi(x, c)}[r(\xi)]$ for $c \in \mathcal{C}$.
% % We first note that if the human never makes mistakes, then the choice of $\hat{\beta}$ does not matter.
% \begin{proposition}
% If the human is optimal, then $r^*$ is an MLE estimate for any value of $\hat{\beta} \in [0,\infty)$.
% \end{proposition}
% \begin{proof}
% An optimal human (i.e., $\beta = \infty$) never makes mistakes. Thus, $r^*(c_h) \geq r^*(c), \forall c \in \mathcal{C}$ and
% \begin{eqnarray}
% r^* \in \arg \max_r e^{  r(c_h)} = \arg \max_r e^{\hat{\beta} \cdot  r(c_h)} = \arg\max_r P(c_h | r, \hat{\beta}).
% \end{eqnarray}
% Thus, $r^*$ is an MLE estimate given $c_h$, $\forall \hat{\beta} \in [0, \infty)$.
% \end{proof}

% Even though the MLE reward may not change, the shape of the posterior distribution over $r$ is strongly influenced by the choice of $\hat{\beta}$. When the human is suboptimal, we want to have robots that hedge their bets, rather than becoming overly confident in their estimate of the true reward function.
% Jonnavittula and Losey~\cite{jonnavittula2021know} propose using
% the Shannon entropy over the robot’s belief $P(r \mid c_h)$ as a measure of the risk-aversion of a robot.  Using this definition of risk we have the following result. 

% \begin{proposition}
% The robot becomes less risk-averse as $\hat{\beta}$ increases.
% \end{proposition}
% \begin{proof}
% If $\hat{\beta} =0$, then we have a uniform belief distribution over $r$, resulting in maximum entropy and risk-averse behavior. As $\hat{\beta}$ increases, the posterior distribution concentrates on only a small number of reward functions $r$, resulting in lower entropy and less risk-aversion. To see this note that
% \begin{eqnarray}
%     P(r \mid c_h) &\propto& \frac{\exp(\hat{\beta} \cdot r(c_h))}{\sum_{c \in \mathcal{C}} \exp (\hat{\beta} \cdot r(c))} P(r)
%     = \frac{1}{1 + \sum_{c \neq c_h} \exp (\hat{\beta} \cdot \left( r(c) - r(c_h)) \right)} P(r)
% \end{eqnarray}
% As $\hat{\beta} \rightarrow \infty$, we have $\exp (\hat{\beta} \cdot \left( r(c) - r(c_h)) \right) \rightarrow 0$ if $r(\varphi(x,c)) < r(c_h)$ and $\exp (\hat{\beta} \cdot \left( r(c) - r(c_h)) \right) \rightarrow \infty$ if $r(\varphi(x,c)) > r(c_h)$. Thus, $P(r \mid c_h, x, \mathcal{C}, \varphi, \hat{\beta}) \rightarrow 0$ as $\hat{\beta} \rightarrow \infty$ if $c_h$ does not maximize $r(c)$ and $P(r \mid c_h, x, \mathcal{C}, \varphi, \hat{\beta}) \propto 1$ if $c_h$ uniquely maximizes $r(c)$. If $c_h$ is a non-unique maximizer of $r(\phi(x,c))$, then we have $P(r \mid c_h, x, \mathcal{C}, \varphi, \hat{\beta}) \propto 1/|\{c : r(c) = r(c_h) \}|$. 
% % Thus, the posterior belief distribution entropy decreases as $\hat{\beta}$ increases and concentrates only on rewards $r$ such that $c_h$ is a maximizer of $r(\phi(x,c))$.
% % and the entropy goes to zero if $c_h$ is the unique optimal choice.
% \end{proof}
% As a consequence, we have the following result about suboptimal behavior due to bias or noise.

% \begin{proposition}
% If the human makes a mistake, then the likelihood of the true reward, $r^*$, decreases exponentially as $\hat{\beta}$ increases.
% \end{proposition}
% \begin{proof}
% For a suboptimal choice $c_h$, $\exists c^* \in \mathcal{C}$ such that $r^*(c_h) < r^*(c^*)$ and 
% \begin{equation}
%     P(c_h | r^*, \hat{\beta}) = \frac{\exp(\hat{\beta} r^*(c_h))}{\sum_{c} \exp(\hat{\beta} r^*(c))} < \frac{\exp(\hat{\beta} r^*(c_h))}{\exp(\hat{\beta} r^*(c^*))} = \exp(\hat{\beta} (r^*(c_h) - r^*(c^*))).
% \end{equation}
% By assumption, $r^*(c_h) - r^*(c^*) < 0$. Thus, the likelihood decreases exponentially as $\hat{\beta}$ increases.
% \end{proof}

% The above analysis supports our empirical findings and shows that overestimating $\hat{\beta}$ can have negative consequences since it makes the robot overly confident in the human data, potentially overfitting to suboptimialities, whereas using a lower $\hat{\beta}$ leads to more risk-averse behavior (beneficial when the human is suboptimal), while still being optimal (under a uniform prior) when learning from perfectly rational humans.


\section{Reward Inference for Simulated Biased Human Feedback}\label{app:sim_bias_other_metrics}
In the main text of the paper, we have explored the performance of reward inference on simulated-biased demonstrations. Here, we examine the case of a simulated bias for comparisons and e-stops. In the discussion that follows, it is important to observe that different feedback types are varyingly impacted by different biases. One illustrative case of this is biases which affect the perception of the transition dynamics. Such biases would clearly be expected to impact demonstrations because demonstrations rely upon planning a trajectory through the environment. On the other hand, when confronted with the task of comparing two trajectories having already taken place, transition dynamics play no role in computing the Boltzmann rational choice. Notably, this observation plays an important role in motivating the importance of modelling irrationality. If it is possible for a robot to identify that a human's bias has no impact on a particular feedback type, it has the opportunity to select for that feedback type. In this case, we specifically analyze the case of myopia bias and we leave further analysis of the systematic biases affecting other feedback types to future work.
\paragraph{Multiple Biases} We tested the effect of fitting $\beta$ when there are multiple biases simultaneously for Demonstrations. In particular, we examined the case of a simultaneous myopia and extremal bias with parameters (0.5, 0.5). We found that found that \textbf{Default} achieved regret \textbf{0.37±0.12}, \textbf{Fitted} achieved \textbf{0.11±0.08}, and \textbf{Oracle} achieved \textbf{0.05±0.10}.

\subsection{Comparisons}
\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/figs/Appendix_MyopicComp.png}
         \caption{Comparison}
         \label{subfig:app_myopia_comp}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/figs/Appendix_estop_myopic.png}
         \caption{E-Stop}
         \label{subfig:app_extremal_comp}
     \end{subfigure}
    % \hfill
     %\begin{subfigure}[b]{0.24\textwidth}
    %     \centering
    %    \includegraphics[width=\textwidth]{NeurIPS/figs/determinism_bias.png}
     %    \caption{Determinism}
     %    \label{subfig:determinism}
     %\end{subfigure}
     %\hfill
     %\begin{subfigure}[b]{0.32\textwidth}
      %   \centering
      %   \includegraphics[width=\textwidth]{NeurIPS/figs/Optimism.png}
     %     \caption{Optimism}
     %    \label{subfig:optimism}
     %\end{subfigure}
        \caption{ \textbf{Reward Inference on Simulated Biased Comparisons and E-Stops.} We compare the $\beta$-fitting method (\textit{Fitted}) introduced in this work with a \textit{Default} method which assumes $\beta=1$ and an \textit{Oracle} method that performs reward inference with access to a perfect model of the biased human. We see in (a) that $\beta$-fitting improves reward inference in the case of comparisons. However, in (b), we find that $\beta$-fitting does not improve performance very much in the case of E-Stops.
        }
         \label{fig:biasedfeedbackcomp}
\end{figure*}
 Recall that the observation model for Boltzmann-rational comparisons as shown in Equation \ref{comp_eq}, involves the quantity $r(\xi) = \sum_{(s,a) \in \xi} r(s,a)$, the cumulative reward achieved during the trajectory. In order to simulate Myopia bias for comparisons, we introduce a discount factor $\gamma$ into this cumulative reward calculation and simulate the comparison choices to be Boltzmann-rational with respect to the discounted cumulative rewards. In Figure \ref{fig:biasedfeedbackcomp} (a), we display the impact of $\beta$-fitting for these biased comparisons. We find that there exists a narrower range of $\gamma$ under which the reward can be recovered well even by the oracle method. Nevertheless, on this range we find the $\beta$-fitting results in substantial improvements to the reward inference.
\subsection{E-Stops}
In order to simulate myopic e-stops, we multiplied a discount factor to the accumulated reward used in the observation model for Boltzmann-rational E-Stops. In Figure \ref{fig:biasedfeedbackcomp} (b), we examine the impact of $\beta$-fitting on myopic e-stops, finding that $\beta$-fitting provides a slight, but not significant improvement over the default method. 




\section{Information Gain Crossover Example}
\label{sec:crossover-example}
\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{NeurIPS/figs/Appendix_post_ent.png}
\caption{\textbf{Example of Posterior Mean Entropy of Comparisons and Demonstrations}. We plot the expected posterior entropy after using comparisons or demonstrations for the example presented in Section E. We observe that there is a sharp transition around $\beta = 1$ from comparisons providing the largest reduction in entropy to demonstrations. We examine the intuition of this phenomena in terms of the particular choice sets involved in Section E.}
\end{figure}
Here is a simple environment determined by a few parameters where different settings of the parameters change whether demonstrations or comparisons are more informative, lending some insight into aspects of the environment which favor different feedback types. The set of possible reward parameters is $\Theta = \{\theta_1^+, \theta_1^-, \dots, \theta_N^+, \theta_N^-\}$, the set of possible choices is $\mathcal{C} = \bigcup_{i=1}^N \{c_i^+, c_i^-, c_i^{p_1}, \dots, c_i^{p_K}, c_i^{n_1}, \dots, c_i^{n_K}\}$, and the rewards of each choice depending on the value of the reward parameter are
\begin{align*}
    r(c_i^s, \theta_j^{s'}) &= \begin{cases}
    R_1 & i=j, s=s' \\
    -R_1 & i=j, (s = +, s' = -)\text{ or }(s = -, s' = +) \\
    R_2 & i=j, (s = p_\ell, s' = +) \text{ or }(s = n_\ell, s' = -)\\\MoveEqLeft\text{ for some $\ell$} \\
    -R_2 & i=j, (s = p_\ell,s' = -) \text{ or }(s = n_\ell, s' = +)\\ \MoveEqLeft\text{ for some $\ell$} \\
    R_3 & i \neq j.
    \end{cases}
\end{align*}
We will set $R_1 > R_2 > R_3 > 0$.
Intuitively, the reward has $N$ different "directions," and along a direction $i$ there are two options $\theta^+_i$ and $\theta^-_i$. Supposing that one of $\theta^+_i$ or $\theta^-_i$ are the true reward parameter, then there are $2(K+1)$ choices which are "sensitive" to whether the reward is $\theta^+_i$ versus $\theta^-_i$, while the remaining $(N-1)2(K+1)$ choices all have equal value either way. Among the $2(K+1)$ choices which are sensitive to $\theta^+_i$ versus $\theta^-_i$, there are two extreme options $c_i^+, c_i^-$ which give large reward $R_1$ if they "match" the reward parameter, and very large cost $-R_1$ if they do not match. There are also a larger number $2K$ of "conservative" options which give smaller reward $R_2$ if they match the reward parameter but also less severe cost $-R_2 $ if they do not match the reward parameter.

Now we analyze the expected information gains from human demonstrations and comparisons in this environment. Demonstrations will allow the human to make any choice, while comparisons will present the human with only two choices. We will only analyze comparisons of the form $c_i^+$ vs $c_i^-$ (for some $i$), but this is hardly a limitation because the resulting information gain provides a lower bound on the information gain of the best comparison. We assume a uniform prior over reward parameters in $\Theta$, and for computational convenience we note that maximizing expected information gain is equivalent to minimizing expected posterior entropy, so we can compute expected posterior entropies for demonstrations and comparisons.

First we compute the expected posterior entropy of a demonstration. After observing a choice $c_i^s$, the posterior mass on $\theta_j^{s'}$ is
\begin{align*}
    P(\theta_j^{s'} \mid c_i^s) & \propto P(c_i^s \mid \theta_j^{s'}) \\
    &\propto \begin{cases}
    \exp \beta R_1 & C_{1} \\
    \exp -\beta R_1 & C_{2} \\
    \exp \beta R_2 & C_{3} \\
    \exp -\beta R_2 & C_{4} \\
    \exp \beta R_3 & i \neq j.
    \end{cases}
\end{align*}
    $C_{1}: i=j, s=s'\\ 
    C_{2}: i=j, (s=+, s'=-)\text{ or }(s = -, s' = +)\\
    C_{3}: i=j, (s=p_\ell, s'=+) \text{ or }(s=n_\ell, s'=-)\text{ for some } \ell\\
    C_{4}:i=j, (s=p_\ell, s'=-) \text{ or }(s=n_\ell, s'=+)\text{ for some } \ell\\
    $
    
For $2(N-1)$ values of $\theta_j^{s'}$, we will be in the bottom case, and there will only be two values of $\theta_j^{s'}$ for which we are in any of the top four cases. If $c_i^s$ was an extreme choice $c_i^+$ or $c_i^- $ then we will reach the top two cases each once, otherwise we will reach cases three and four each once. Therefore if one of the extreme options $c_i^+$ or $c_i^- $ was taken, using $H(p_1, \dots, p_k)$ to denote the entropy of a distribution proportional to $(p_1, \dots, p_k)$, we will obtain posterior entropy $$H\bigl(\exp(\beta R_1), \exp(-\beta R_1), \underset{2(N-1)}{\underbrace{\exp(\beta R_3), \dots, \exp(\beta R_3)}}\bigr).$$
If $c_i^s$ was a conservative choice in $c_i^{p_1}, \dots, c_i^{p_K}, c_i^{n_1}, \dots, c_i^{n_K}$ then the posterior entropy will be
$$H\bigl(\exp(\beta R_2), \exp(-\beta R_2), \underset{2(N-1)}{\underbrace{\exp(\beta R_3), \dots, \exp(\beta R_3)}}\bigr).$$
The probability of the human choosing an extreme choice is proportional to $\exp(\beta R_1) + \exp(-\beta R_1) + 2(N-1)\exp(\beta R_3)$ and the probability of choosing a conservative choice is proportional to $K \exp(\beta R_2) + K  \exp(-\beta R_2) + 2K(N-1) \exp(\beta R_3)$. (Adding these two quantities provides the normalizing constant.) These calculations combine to yield the expected entropy of the human posterior after providing a demonstration.

Now we compute the expected posterior entropy after a comparison. Again, instead of computing the expected posterior entropies of all comparisons and using the best, we only consider comparisons of the form $c_i^+$ vs $c_i^-$, where $i$ is fixed. WLOG we can assume that $c_i^+$ is chosen (since the posterior in the case that $c_i^-$ is chosen is the same up to permutation). The posterior mass on $\theta_j^s$ is
\begin{align*}
    P(\theta_j^s \mid c_i^+) &\propto P(c_i^+ \mid \theta_j^s) \\
    &\propto \begin{cases}
    \exp(\beta R_1) / Z & i=j, s=+  \\
    \exp(-\beta R_1) / Z & i=j, s=- \\
    1/2 & i \neq j
    \end{cases}
\end{align*}
where we define $Z = \exp(\beta R_1) + \exp(- \beta R_1)$. Therefore the posterior entropy is
$$H\bigl(\exp(\beta R_1)/Z, \exp(-\beta R_1)/Z, \underset{2(N-1)}{\underbrace{1/2, \dots, 1/2}}\bigr).$$

We now provide more intuition into these calculations. When an "extreme" choice is taken by the human for a demonstration, we obtain the posterior with the lowest entropy. However, as $K$ increases, it becomes more likely that the human will instead take one of the (less rewarding but more numerous) "conservative" demonstration choices, which result in a worse posterior. This provides an opportunity for comparisons to have a lower expected posterior entropy since the comparison is between some two extreme options $c_i^+$ and $c_i^-$, thus eliminating the conservative and less informative choices. However, for comparisons to be more informative, we need $N$ to be sufficiently low (depending on the values of the other parameters, including $\beta$). This can be verified by examining the entropies calculated above, but an intuitive explanation is that a comparison can only present the two options $c_i^+$ and $c_i^-$  for one particular value of $i$, but the correct value of $i$ (matching the $j$ such that $\theta_j^s$ is the human's reward parameter) to ask for is not known and thus there is only a $1/N$ chance that the robot guesses correctly, and the rest of the time the robot must be presenting the human two options towards which the human is completely indifferent. The robot knows this and thus must temper the formed posterior. When $N=1$ and $K>0$, comparisons are actually strictly superior to demonstrations (for all $\beta$), since the comparison is removing the conservative options and thus forcing the human to make a more informative choice, without being penalized for possibly missing the important direction $i$. When $N>1$, keeping all other parameters fixed, whether demonstrations or comparisons are superior may depend on $\beta$, since it depends on which effect is more harmful: high "dimensionality" causing a large probability of a comparison asking about an irrelevant reward direction, or large $K$ and low $\beta$ causing a large probability of a provided demonstration making a choice which is suboptimal and thus results in a higher-entropy posterior.



%\subsection{Extra Writing}
%%Etixisting writing%%
%Setting aside the simplifying assumption, the quality of human feedback will likely vary across feedback types, as a function of the human's abilities as well as features of the environment which affect the relative difficulties of the different feedback types. Therefore the ability of the robot to ask for multiple types of feedback may allow it to adapt to the strengths of the human demonstrator and perform the most effective reward inference. This experiment attempts to better understand the relative informativeness of different feedback types as a function of the human's abilities for each type as well as the environment. First we randomly selected the human's preferences. Then for each level of beta and for each feedback type, we computed the maximum (over designs possible for the feedback type) expected information gain of one sample from the human, assuming that the robot had a flat prior over the human's possible preferences. We plotted these values for multiple environments.

%Surprisingly, in all environments, there were beta levels at which all feedback types had (approximately) the same informativeness. This observation does not have an immediate implication for the optimal feedback type to query, because the demonstrator almost certainly will have different beta levels for each different type and also because the relative informativeness of different types may still change (as we will see in later experiments?) after one sample (again, the expected information gains in these plots assume that no samples have yet been taken from the human). Still, it is surprising that such crossover points exist: even if the demonstrator is "equally good" at providing each feedback type, if this ability level is sufficiently low, then it is better to ask for feedback types that involve comparisons between fewer options.

%A higher-level takeaway is that the relative informativeness of different feedback types depends strongly on the values of beta for all feedback types, so an active learner with knowledge of these beta values may outperform an active learner which does not attempt to estimate beta.

%In this section, we seek to understand the reasons that $\beta$-fitting may succeed or fail to model a particular bias well enough to improve reward inference. We examine two important assumptions (1) the learned rationality parameter $\hat{\beta}$ generalizes well across different reward functions and (2) Boltzmann-rationality, with a tuned $\hat{\beta}$, can approximate the bias.
% \paragraph{Exact Beta Inference}
%To remove sampling errors, in the following analysis, we consider the infinite data case for fitting $\hat{\beta}$. See Appendix~\ref{app:exact_beta_inf} for details.
%\dbnote{Matthew or Gaurav, can you maybe add another sentence or two about this?}


%\paragraph{Beta Generalization} We first analyze how well $\hat{\beta}$ fit from biased human feedback for one calibration reward $r'$ generalizes to other reward functions. For this resulting beta estimate $\hat{\beta}$ to be useful for reward inference on the true reward $\theta^\star$, the human feedback should appear to have a similar level of rationality when optimizing for $r^\star$ as when optimizing for $r'$.
%In \figref{subfig:myopia_beta_spread} and \figref{subfig:optimism_beta_spread} we examine the distribution over $\hat{\beta}$ when fitting with different calibration rewards $r'$ for the same level of bias. We find that \dbnote{@Gaurav: TODO ........................}. 
% We examine the variance of the fitted beta under one bias that we observe improved reward inference results (Myopia) and one bias for which beta-fitting does not yield improvements (Optimism) when learning from demonstrations. The results are shown in \figref{} \textbf{TODO: add results for beta generalization.}. We find that \textbf{TODO: does it work?}. 
%See Appendix~\ref{app:exact_beta_empirical} for an analysis of the other biases and other feedback types. 

% \paragraph{Quality of Fit}
% \begin{figure}
%     \centering
%     \includegraphics[width = \textwidth]{UAI/Figures/5.2.2 IdentifiabilityQualityofFit/Untitled-2.png}
%     \caption{\textbf{KL Divergence between Biased Demonstration Policy and Boltzmann Optimal Trajectories.} Add description of main takeaways .....}

    
%     \label{fig:kldivergence}
    
% \end{figure}





%\dbnote{@Gaurav: I'm not sure where this paragraph should go. Is it different from the identifiability or can we merge it with the next paragraph?}
%For our proposed $\beta$-fitting method to work, we need to be able to approximate biased behavior with Boltzmann rational behavior with a specific $\beta$ parameter. The approximation error can be quantitatively measured as the KL-Divergence between the biased demonstration policy and the Boltzmann-rational demonstration policy of the ground truth reward $\theta$, as is marked by the horizontal black lines in \figref{fig:kldivergence}. We observe that that for Myopia, the KL-Divergences are uniformly low across a range of $\gamma$ parameters, suggesting that Myopic behavior is modelled very well by Boltzmann rationality. On the other hand, we see that for certain parameter values of optimism, the magnitude of KL-divergence is very high, suggesting a poor fit. 


%\paragraph{Identifiability of Reward} \dbnote{@Gaurav can you work on trimming this down and refer to the specific subfigures in the discussion?} We can see that magnitude of KL-Divergence does not fully explain when $\beta$-fitting works. As an example, when the Myopia $\gamma = 0.1$, the KL-Divergence metric is close to 0 according to \figref{fig:kldivergence}(b), but fitted inference performs much worse than oracle. To investigate this, we compute the KL-Divergence between the biased demonstration policy and Boltzmann rational policies corresponding to every other candidate reward function. This is shown in \figref{fig:kldivergence}, where each point represents a candidate reward. In the cases where our method performs worse than oracle, all candidate reward functions have very similar KL-Divergences to our biased behavior. This suggests that all reward functions roughly explain the biased behavior equally well, so it is difficult to identify the true reward from all the others. On the other hand, in cases where our method works comparably to the oracle, the candidate reward functions are spread out in their KL-Divergence to the biased policy.

\section{Exact Beta Inference}
\label{app:exact_beta_inf}

\subsection{Demonstrations}
When there is access given to the underlying demonstration policy, it is possible to conduct exact inference of the human's rationality.
Because we have access to the entire policy (for a given $\theta$) $\pi$ describing the simulated biased demonstrators, we can circumvent forming $\beta$ estimates by sampling from $\pi$ by instead performing an exact M-projection of $\pi$ onto the family of softoptimal policies $\{\pi_{\beta, \theta} :  \beta \in (0, \infty)\}$ for the particular reward $\theta$:
\begin{align*}
    \hat{\beta} &= \argmin_{\beta \in (0, \infty)} D_{KL}(\pi \mid \mid  \pi_{\beta, \theta}) \\
    &= \argmin_{\beta \in (0, \infty)} \sum_{\xi} \pi(\xi) \log \left( \frac{\pi(\xi)}{\pi_{\beta, \theta}(\xi)}\right) \\
    &= \argmin_{\beta \in (0, \infty)} \sum_{\xi} \pi(\xi) \left( \sum_{t = 0}^{T-1}\log \left( \frac{\pi(a_t \mid s_t)}{\pi_{\beta, \theta}(a_t \mid s_t)}\right) \right) \\
\end{align*}
and the term inside the $\arg \min$ can be evaluated efficiently because it is equivalent to policy evaluation of the policy $\pi$ on the non-stationary reward $r_t(s, a) = \log(\frac{\pi(a_t \mid s_t)}{\pi_{\beta, \theta}(a_t \mid s_t)})$. This is an optimization problem over a single scalar variable so it is easy to solve.


\subsection{Comparisons and E-Stops}
For comparisons and E-stops we take the same approach of performing exact M-projection, but in these cases this is simpler to compute due to the much smaller number of possible choices. We describe this in slightly more generality and then specialize to comparisons and E-stops.

Given $m$ choices $c_1, \dots, c_m$ with rewards $r_{1, \theta}, \dots, r_{m, \theta}$, we can define the $\beta$-rational policy (for a particular $\theta$) $\pi_{\beta, \theta}$ to be the policy which makes choice $c_i$ with probability 
$\exp(\beta r_{i, \theta})/{\sum_{j=1}^m \exp(\beta r_{j, \theta})}$. A general human can be described by the policy $\pi$ which specifies the probabilities of taking each choice. To compute the M-projection we evaluate $
    D_{KL}(\pi \mid \mid  \pi_{\beta, \theta})
$
by simply expanding its definition. This applies to comparisons by taking $m=2$ and to E-stops by having the choices as $c_1, \dots, c_m = \xi_{0:0}, \dots, \xi_{0,T}$ for some trajectory $\xi$. As described this only accommodates a single design (ex. one pair of trajectories to compare/one trajectory to stop along) but the extension to multiple designs is immediate since the choice taken in each design is independent and thus the KL divergence between the true model and a $\beta$-rational model for multiple choices in multiple designs is simply the sum of the individual KL-divergences for each design.


\section{Exact Beta Inference Empirical Results}\label{app:exact_beta_empirical}
\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/figs/Appendix_extremalkl.png}
         \caption{KL Divergence}
         \label{subfig:app_kl_myopia}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/figs/Appendix_ExtremalVariance.png}
         \caption{Beta Variance}
         \label{subfig:app_var_extremal}
     \end{subfigure}
        \caption{ \textbf{Exact Inference Analysis for Extremal Bias}. In (a), we show the KL-Divergence of extremal-biased policies against all Boltzmann-rational policies across the candidate reward functions. Our results reinforce the ideas of reward identifiability introduced in the main paper, as the settings where $\beta$ fitting performs comparably to oracle are when the KL-divergences are very spread out. In (b), we show the variance of $\hat{\beta}$ across all reward functions as a measure of $\beta$ generalization. Our variance results do not fully explain the success or failure of $\beta$-fitting because the variance is uniformly low across all bias levels.}
         \label{fig:klextremal}
\end{figure*}
In the main text of the paper, we presented some analysis of the generalization of $\beta$ and the reward identifiability for the myopia and optimism biases. Here we provide a similar analysis for the extremal bias. In Figure \ref{fig:klextremal} (a), we show KL Divergence between the extremal-biased policy and Boltzmann-rational policies for every other candidate reward function. We find that at extremal bias levels where the KL Divergences are spread out, our fitted method performs comparably with the oracle method. On the other hand, at $\alpha$ values where all reward functions have roughly the same KL-Divergence, we find that the fitted method performs worse than oracle. This gives further evidence for the concept of reward identifiability presented in the paper. Additionally, in Figure \ref{fig:klextremal} (b), we presented the variance of $\hat{\beta}$ over all the reward functions at at different levels of extremal bias. We observe that the magnitude of $\beta$ variance is uniformly low. However, we observe the slightly counter-intuitive result that at the parameter values where the $\beta$ variance is lowest, our method does not perform as well as Oracle, showing that the generalization ability of $\beta$ across different reward functions is insufficient to explain the success or failure of $\beta$ fitting. 
\section{Impact of Assumed \texorpdfstring{$\beta$}{Beta} on Learning From a Biased Human}
\textcolor{blue}{\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/figs/Appendix_Beta0.5Myopia.png}
         \caption{$\beta=0.5$}
         \label{subfig:app_myopia}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/figs/Appendix_Beta5Myopia.png}
         \caption{$\beta=5$}
         \label{subfig:app_extremal}
     \end{subfigure}
        \caption{ \textbf{Varying Default Assumed $\beta$}. In this figure, we examine reward inference for myopic demonstrations in the case where the default $\beta$ is considered be (a) 0.5 or (b) 5. We find that increasing the assumed $\beta$ causes the default method to perform worse in comparison to fitted and oracle, while decreasing it narrows the gap between the methods.
        }
         \label{fig:betadefaultvary}
\end{figure*}}

In Figure \ref{fig:betadefaultvary}, we examine the effect of assuming different default $\beta$ values when learning from myopic demonstrations. In one case, we decreased the assumed $\beta$ to 0.5 and found that this caused the default method to perform more comparably to fitted and oracle. In another case, we increased the assumed beta to 5. We found that this caused the default method to perform even more poorly relative to fitted and oracle. These results give further evidence for the theory presented in Section 3: Reducing the assumed $\beta$ causes default to \textit{overestimate} less, leading to improved reward inference. On the other hand, when we increase the assumed $\beta$, default overestimates the true $\beta$, leading to worse reward inference.
\section{Additional Active Learning Ablations}

\begin{figure*}
\centering
\label{fig:secondablation}
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/figs/Appendix_SecondAblationStudy.png}
         \caption{$\beta_{default}=10, \beta_{demo}=1$}
         \label{subfig:app_additional_al_1}
     \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/figs/Appendix_Ablation_2.png}
         \caption{$\beta_{default}=10, \beta_{comp}=1$}
         \label{subfig:app_additional_al_2}
     \end{subfigure}

\caption{\textbf{Additional Active Learning Ablation}. In (a) We additionally consider an active learning ablation in the case that demonstrations are the most rational feedback type and the assumed $\beta$ over-estimates the rationality of every feedback type. In this case, we find that have the correct reward inference beta plays a role of increased importance. In (b), we consider the case where the default $\beta$ overestimates the true rationality and comparisons are the most rational feedback type. Here, we observe that while having the correct active learning $\beta$ is very important (so that you know to choose comparisons), having the correct reward inference beta plays a larger role than the result shown in Figure 4(b), since the default rationality in this case over-estimates the feedback rationality, as opposed to under-estimating it (as is the case in 4(b).}
\end{figure*}
In addition to the active learning setting provided in the main text, we also analyzed the case where (a) the default $\beta$ over-estimates the all true rationalities and (b) the relative rationalities of different feedback types are changed. In order to conduct this study, we set the assumed $\beta$=10 and the true $\beta_{demo}=1, \beta_{comp}=0.5, \beta_{estop}=0.1$. The results are shown in Figure 10. In this case, we find that having the correct $\beta$ for reward inference plays a larger role in determining the performance of the active reward inference. We attribute this to the fact that when the default rationality is used for reward inference, demonstrations are primarily still selected. However, the $\beta=10$ in reward inference severely overestimates the true rationality which causes reward inference to be poor. In Figure 11 (b), we consider the case where the default over-estimates all feedback rationalities and the most informative feedback type is comparisons. In this case, having the correct active learning beta is very important, as this is necessary to correctly choose comparisons queries. However, we see that not having the correct reward inference beta also leads larger to reductions in performance than seen in Figure 4(b). This can be explained by the fact that using the default reward inference rationality in this case causes an overestimation of the feedback rationality, which as shown by our theory can be harmful.

\section{User Study Details}

The user study was performed according to IRB approval and consent was obtained by having the participant review and ask questions about a consent form prior to the study taking place. All data collected from each participant was anonymized. Participants were compensated for their time at a rate of 20 dollars an hour. The user study was designed to take approximately 45 minutes and participants received no less than 15 dollars regardless of the amount of time it took them to complete the study.  In total, \$105 was spent on participant compensation.
\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/figs/Appendix_DemoCollector.png}
         \caption{Demonstrations}
         \label{subfig:app_user_demo}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.6\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/figs/Appendix_CompInterface.png}
         \caption{Comparisons}
         \label{subfig:app_user_comp}
     \end{subfigure}
        \caption{ \textbf{User Study Interface}. We show the feedback collection interface for demonstrations (a) and comparisons (b). For demonstrations, the participants could view in real-time the position of the agent, their current score, and the time step. When providing comparisons, participants had access to a trace of the trajectory in the environment, as well as the counts of how many time-steps the agent spent in each colored tile.  
        }
         \label{fig:userstudyinterface}
\end{figure*}

In our user study, we presented 5 calibration rewards to each user (using the interface shown below) and asked them to provide 10 instances of feedback per reward (5 comparisons and 5 demonstrations). In Figure \ref{fig:userstudyinterface}, we provide examples of the feedback collection interfaces for each feedback type. For both feedback types, the reward function was displayed in the top-left hand corner, as a mapping between tile colors and the rewards earned for stepping on the relevant tiles. In addition, there was a completion reward present in the environment of 250 reward and users were advised of this during the instructions phase of the study. The completion reward was chosen to ensure that the optimal path ended in the goal state, while also ensuring that the shortest path from start to goal was not always optimal. 
\paragraph{Demonstration Interface}  Figure \ref{fig:userstudyinterface} (a) shows the demonstration collection interface. In addition to the reward function, participants were provided with real-time access to the current reward score achieved by the demonstration, as well as the current time step. The agent's position was depicted by the black circle and the participant was able to control its movement by using the arrow keys. Participants experienced time pressure when giving the demonstration, as the interface ran at 6 time-steps per second and failure to provide control input at a given time-step would result in the agent continuing to slide in its last direction of movement. The participant was given unlimited time to review the reward function and starting state prior to beginning the demonstration and would press the A key to start the demonstration. 
\paragraph{Comparisons Interface} The participant was presented with two trajectories and asked to compare which was superior under the given reward function. To assist them in making their decision, they were provided with environment maps depicting a trace of the agent's movement. Moreover, participants were provided with time-step counts of how long the agent spent in each color tile. Participants were allowed unlimited time and could indicate their selection by pressing 1 to select the left trajectory and 2 for the right. 

Prior to beginning, participants were provided with the following instructions:

\textit{In this user study, you will be providing two different feedback types to help an artificial intelligence agent infer a reward function. You will be providing demonstrations and comparisons.}


\textit{You will be providing feedback in a 10x10 gridworld environment, where the tiles have four possible colors. You will be controlling the orange circle when you give your demonstrations. 
Each reward function will be a mapping between tile colors and a reward you get for every time step you spend on the tile color. 
The environment will have a horizon length of 25. This means that the maximum number of steps in a trajectory is 25. }

\textit{The black square in the bottom right corner of the environment is a goal state. Provided you reach the goal state by the end of the horizon, you will receive +250 reward. If you arrive at the goal before the horizon ends, you will receive +250 reward at the point you reach the goal and +0 reward for all future time steps.
You will provide demonstrations using an interface that looks like the above. You will control the movement of the agent using the arrow keys (up key moves up, down key moves down, left key moves left, right key moves right). You will experience time pressure when giving demonstrations. The interface will run at 6 time-steps per second and if you don’t provide input at a given step, the agent will slide in the direction it was last moving. 
Score: The score field on the left-hand side will tell you the current score you have accumulated 
Step: The step field on the right-hand side will tell you how many time-steps have elapsed since the beginning of the episode.}

\textit{You are encouraged to review the reward function carefully before starting the demonstration. When you are ready to begin, you should press the “a” key and then begin controlling the robot.
You will also be providing preference comparisons between two trajectories that the robot itself has generated.A trace of the trajectory is shown on the screen. We have also provided information about how long the robot spends on each color to help you decide which trajectory better represents the reward.
}

Following the presentation of the instructions, the participant was given unlimited practice attempts on each feedback type. They were also given a chance to ask any questions they ha about the interface or the strategy for giving the feedback. After this, the participants began the formal study. 

Participants first provided 25 demonstrations, followed by 25 comparisons. The feedback of each type was provided in 5 blocks of 5, where each block consisted consisted of the same reward function. In between blocks, the interface alerted the participants to the fact that the reward function had changed. Since participants had unlimited time to review the reward function before providing a demonstration or indicating a comparison, they were able to pace themselves and take breaks as necessary.

We used a hold-one-out method for analyzing the user study data. In this setting, we would test reward inference on each reward function by fitting beta on the data provided for the other 4 reward functions and then testing the reward inference on the held-out reward function. We completed this for each reward function, resulting in 5 trials per user.
\paragraph{Statistical Tests} We also conducted a two-tailed paired T-Test between the fitted and default reward inference results computed in the User Study. The results are shown in Table 3 and demonstrate that, while there was a statistically significant difference for both active learning and demonstrations, we did not observe a statistically significant difference between the methods for comparisons.
\begin{table*}
\label{tab:app_t_test}
\footnotesize
\centering
    \caption{User Study t-test Results.}\label{tab:userstudyttest}
\begin{tabular}{llll}
 \toprule % from booktabs package
\bfseries Feedback Type  & \bfseries p-Value   \\
 \midrule % from booktabs package
            %   &                                & for $x \in \mathcal{X}$                        & for $x \in \mathcal{X}, c \in \mathcal{C}(x)$                                           \\
% Demonstration (old) & Starting states:               & Trajectories:                  & $\varphi(s, \xi) = \xi$    \\
%               & $\mathcal{X} = \mathcal{S}$    & $\mathcal{C}(s) = \{\xi \in \Xi : \xi_0 = s\}$ &                                                                                         \\
% \midrule
              
Demonstration & 0.02                                                               \\
              
\midrule % from booktabs package

Comparison & 0.34 \\

\midrule % from booktabs package
Active  & 0.0001                
\end{tabular}
% \adnote{comparisons -- any two trajectories, or any two trajectoires that start at the same state?; stopping time: the trajectory stays stopped after t, so it repeats xi(t) until the end of the horizon but has the same length, right?;  }

% \dbnote{I don't think there is anything in our formalism requires the trajectories to start from the same point. Our version of e-stops doesn't repeat the stopped state but just ends the episode upon an e-stop.}
\end{table*}
\begin{figure*}
\centering
      \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/figs/CarDriving.png}
         \caption{Environment Visualization}
         \label{subfig:app_car_inter}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/figs/CarDrivingMyopia.png}
         \caption{Myopia}
         \label{subfig:app_car_myopia}
     \end{subfigure}
     \hfill
    \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/figs/CarDrivingExtremal.png}
         \caption{Extremal}
         \label{subfig:app_carextremal}
     \end{subfigure}

\caption{\textbf{Car Driving Simulator}. In (a), we show a visualization of our car-driving environment. In (b) and (c) we show the performance of modelling rationality in the car driving setting when learning from biased feedback. We find that beta-fitting results in improved reward inference in both the myopia and extremal biased settings.}
\label{fig:car}
\end{figure*}

\section{Car Driving Simulator}
In addition to our results in the gridworld navigation environment, we tested the importance of fitting $\beta$ on a car driving simulator environment we developed. In our simulator, the agent car drives along a three-lane road in the presence of other vehicles. The reward features considered are a car crash indicator, in addition to a one-hot encoded indicator of the cars lane (allowing for a lane preference in the reward function). In Figure~\ref{fig:car}, we show that learning a reward function from biased feedback can be improved by modeling rationality in the way we propose.
\section{Compute Resources Used}
The majority of experiments, as well as the user study for this paper were run on a Mid-2015 MacBook-Pro with an Intel Quad-Core i7 Processor. Certain experiments were run on a lab Intel 8-core i7 Processor.
